GLOBEM Dataset: Multi-Year Datasets for Longitudinal Human Behavior Modeling Generalization

Recent research has demonstrated the capability of behavior signals captured by smartphones and wearables for longitudinal behavior modeling. However, there is a lack of a comprehensive public dataset that serves as an open testbed for fair comparison among algorithms. Moreover, prior studies mainly evaluate algorithms using data from a single population within a short period, without measuring the cross-dataset generalizability of these algorithms. We present the first multi-year passive sensing datasets, containing over 700 user-years and 497 unique users' data collected from mobile and wearable sensors, together with a wide range of well-being metrics. Our datasets can support multiple cross-dataset evaluations of behavior modeling algorithms' generalizability across different users and years. As a starting point, we provide the benchmark results of 18 algorithms on the task of depression detection. Our results indicate that both prior depression detection algorithms and domain generalization techniques show potential but need further research to achieve adequate cross-dataset generalizability. We envision our multi-year datasets can support the ML community in developing generalizable longitudinal behavior modeling algorithms.

==> 1-introduction_old.tex <==
\section{Introduction}
\label{sec:introduction}

The past decade has witnessed a surge of mobile technology advances. Smartphones and wearables have become a part of everyday life.
This provides an unprecedented opportunity for these smart devices to capture various aspects of daily human behaviors, by collecting continuous, longitudinal, passive sensing data streams, such as location trajectory, phone usage, and physical activity.
Recently, researchers have demonstrated the potential of using longitudinal passive sensing data for behavior modeling in many applications, \eg detecting physical health issues~\cite{min2014_10.1145/2556288.2557220}, monitoring mental health status~\cite{wang2014studentlife}, measuring job performance~\cite{mattingly2019tesserae}, and tracing education outcomes~\cite{wang2015smartgpa}.

A typical behavior modeling research starts from conducting a field experiment for passive sensing data collection, to developing behavior modeling algorithms using the dataset~\cite{xu_understanding_2021}.
However, such a methodology has two major limitations.
First, there is a lack of cross-dataset generalization evaluation for a behavior modeling algorithm developed based on a single dataset.
Second, there is a lack of public datasets for standard algorithm evaluation and comparison, as different research groups train and test their models using their own private datasets.

To date, the only public longitudinal passive sensing dataset is from the pioneering StudentLife Study~\cite{studentlife_study_2014}.
However, it only contains 48 students over a 10-week academic quarter. The single dataset within a short time span cannot support a cross-dataset generalization evaluation task (the first limitation).
Meanwhile, the limited sample size can hardly serve as a golden testbed for various behavior modeling algorithms (the second limitation).

To address these limitations, we present our multi-year data collection studies that span four years (10 weeks each year, from 2018 to 2021). Each year's data includes new participants and a small portion of continuing participants (since the second year). Our multi-year dataset contains close to 500 unique users in total (over 700 person-year).
We employ a consistent data collection method: participants install a mobile app on their phone and wear a fitness tracker (Fitbit, provided by us). The app and wearable device passively track multiple sensor streams in the background 24/7, including location, phone usage, call, Bluetooth, physical activity, and sleep behavior. In addition, participants need to fill in several long surveys and weekly short questionnaires to report numerous aspects of their livings, including personality, mental health status, social well-being, \etc\ These survey data can be leveraged as the ground truth for various behavior modeling targets.
Our statistical analysis indicates that our dataset captures a wide range of daily human routines and reveals insights between daily behaviors and important well-being metrics (\eg depression status).
Our dataset can serve as a reliable testbed and support multiple cross-dataset generalization tasks to evaluate a behavior modeling algorithm's generalizability (\eg different users across different years) and robustness (\eg same users over multiple years).

As a starting point, we report benchmark results of a behavior modeling task with depression detection as the target, a binary classification task to distinguish whether participants had at least mild depression using historical passive sensing data.
We closely re-implement 9 prior depression detection algorithms, 8 recent deep-learning-based domain generalization algorithms, and our newly proposed algorithm, \textit{Reorder}.
These 18 algorithms are consolidated on a platform \textbf{GLOBEM} (short for \underline{\textbf{G}}eneralization of \underline{\textbf{LO}}ngitudinal \underline{\textbf{BE}}havior \underline{\textbf{M}}odeling)
\footnote{Although not the major contribution of this work, the platform can be found at \href{https://github.com/anonymized-anonymity/GLOBEM\_review}{https://github.com/anonymized-anonymity/GLOBEM\_review}}.
We evaluate the generalizability of these algorithms with multiple cross-dataset generalization tasks, including leave-one-dataset-out, pre/post COVID, and overlapping users across years.
Our results indicate that these algorithms can barely generalize across datasets. Although our algorithm \textit{Reorder} has the best overall generalizability ($\Delta = 6.6\%$ on balanced accuracy over other algorithms), its advantage is still marginal and far from practical deployability. The community needs more continuous effort to develop better behavior modeling algorithms.

The contributions of this work can be summarized as follows:
1) We present and release our multi-year passive sensing dataset that contains over 600 users' data, including multiple sensor streams and various self-report questionnaire outcomes.\footnote{Due to the sensitive nature of the dataset, we release our data with open credentialed access.}
2) We conduct a series of analyses on our dataset. The results indicate that our passive sensing data capture various daily behavior routines and reveal meaningful behavior insights.
3) We report benchmark results of 17 existing modeling algorithms and one new algorithm on the depression detection task, which shows the advantage of our algorithm, but also suggests the lack of generalizability of all algorithms.
We call for researchers' attention to developing more generalizable longitudinal behavior modeling algorithms.

Our dataset description and example analysis is open-sourced at \href{https://github.com/anonymized-anonymity/GLOBEM-data}{https://github.com/anonymized-anonymity/GLOBEM-data}.

==> fig_tab_alg/fig_dataset_distinguish.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_dataset_distinguish_neurips.pdf}
    \caption{Performance of The Name-The-Dataset Task using A Random Forest (n=10, maximum depth=3).}
    \label{fig:dataset_distinguish}
\end{figure}

==> fig_tab_alg/fig_person_distinguish.tex <==
\begin{figure}[b]
    \centering
    \includegraphics[width=1\columnwidth]{figures/results_person_distinguish_neurips.pdf}
    \caption{Performance of The Distinguish-The-Person Task using A Random Forest (n=10, maximum number of leaves = 2K).}
    \label{fig:person_distinguish}
\end{figure}

==> fig_tab_alg/tab_crossds_display_noref.tex <==
% \renewcommand{\arraystretch}{1.2}
% \begin{table}[t]
% \centering
% \caption{Model Performance of Depression Detection under Different Setups.}
% % \begin{minipage}[t]{0.48\textwidth}
% \resizebox{1\textwidth}{!}{
% \begin{tabular}[t]{c|l|C{0.21\textwidth}|C{0.21\textwidth}|C{0.21\textwidth}|C{0.21\textwidth}}
% \hline \hline
% \multirow{2}{*}{\textbf{Category}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \textbf{Single Dataset} & \multicolumn{3}{c}{\textbf{Cross Dataset}} \\ \cline{3-6}
%  & & \textbf{Past/Future} & \textbf{Leave-One-DS-Out} & \textbf{Pre/Post-COVID} & \textbf{Overlapping Users}\\ \cline{3-6}
% % & & \textbf{Bal Acc}  & \textbf{Bal Acc}  & \textbf{Bal Acc}  & \textbf{Bal Acc}  \\
% \hline
% Baseline & Majority & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} \\ \hdashline
% \multirow{9}{*}{\makecell{Prior\\Depression\\Detection\\Model}} & Canzian \etal & 0.527{\small $\pm$0.027} & 0.495{\small $\pm$0.006} & 0.495{\small $\pm$0.005} & 0.516{\small $\pm$0.018} \\
% & Saeb \etal & 0.554{\small $\pm$0.020} & 0.534{\small $\pm$0.009} & 0.513{\small $\pm$0.002} & {0.561{\small $\pm$0.036}} \\
% & Farhan \etal & 0.570{\small $\pm$0.024} & 0.521{\small $\pm$0.004} & 0.498{\small $\pm$0.032} & 0.476{\small $\pm$0.011} \\
% & Wahle \etal & 0.597{\small $\pm$0.019} & 0.529{\small $\pm$0.014} & 0.527{\small $\pm$0.003} & 0.519{\small $\pm$0.018} \\
% & Lu \etal & 0.552{\small $\pm$0.024} & 0.530{\small $\pm$0.012} & 0.505{\small $\pm$0.011} & 0.501{\small $\pm$0.016} \\
% & Wang \etal & 0.522{\small $\pm$0.014} & 0.517{\small $\pm$0.004} & 0.518{\small $\pm$0.009} & 0.526{\small $\pm$0.028} \\
% & Xu \etal-I & {0.684{\small $\pm$0.017}} & 0.506{\small $\pm$0.011} & 0.512{\small $\pm$0.015} & 0.471{\small $\pm$0.017} \\
% & Xu \etal-P & 0.578{\small $\pm$0.011} & 0.499{\small $\pm$0.007} & 0.507{\small $\pm$0.006} & 0.537{\small $\pm$0.014} \\
% & Chikersal \etal & 0.640{\small $\pm$0.010} & {0.542{\small $\pm$0.010}} & {0.531{\small $\pm$0.019}} & 0.553{\small $\pm$0.032} \\ \hdashline
% \multirow{16}{*}{\makecell{Recent\\Domain\\Generalization\\Model}} & ERM-1dCNN & 0.620{\small $\pm$0.014} & 0.536{\small $\pm$0.007} & 0.535{\small $\pm$0.007} & 0.593{\small $\pm$0.031} \\
% & ERM-2dCNN & 0.560{\small $\pm$0.015} & 0.527{\small $\pm$0.007} & 0.516{\small $\pm$0.006} & {0.597{\small $\pm$0.049}} \\
% & ERM-LSTM & 0.622{\small $\pm$0.008} & 0.532{\small $\pm$0.003} & 0.509{\small $\pm$0.002} & 0.575{\small $\pm$0.026} \\
% & ERM-Transformer & 0.530{\small $\pm$0.005} & 0.521{\small $\pm$0.006} & 0.526{\small $\pm$0.013} & 0.538{\small $\pm$0.006} \\
% & ERM-Mixup & 0.620{\small $\pm$0.014} & 0.542{\small $\pm$0.005} & 0.541{\small $\pm$0.011} & 0.593{\small $\pm$0.031} \\
% & IRM & 0.600{\small $\pm$0.015} & 0.540{\small $\pm$0.013} & 0.537{\small $\pm$0.018} & 0.578{\small $\pm$0.031} \\
% & DANN-D & 0.501{\small $\pm$0.005} & 0.500{\small $\pm$0.000} & 0.507{\small $\pm$0.005} & 0.496{\small $\pm$0.003} \\
% & DANN-P & 0.500{\small $\pm$0.000} & 0.499{\small $\pm$0.001} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} \\
% & CSD-D & 0.612{\small $\pm$0.016} & 0.535{\small $\pm$0.010} & 0.542{\small $\pm$0.007} & 0.582{\small $\pm$0.023} \\
% & CSD-P & 0.609{\small $\pm$0.018} & 0.547{\small $\pm$0.012} & 0.540{\small $\pm$0.006} & 0.577{\small $\pm$0.036} \\
% & MLDG-D & 0.507{\small $\pm$0.016} & 0.516{\small $\pm$0.003} & 0.514{\small $\pm$0.002} & 0.578{\small $\pm$0.033} \\
% & MLDG-P & 0.524{\small $\pm$0.014} & 0.506{\small $\pm$0.004} & 0.515{\small $\pm$0.002} & 0.547{\small $\pm$0.022} \\
% & MASF-D & 0.512{\small $\pm$0.014} & 0.510{\small $\pm$0.009} & 0.498{\small $\pm$0.007} & 0.517{\small $\pm$0.005} \\
% & MASF-P & 0.508{\small $\pm$0.022} & 0.519{\small $\pm$0.004} & 0.507{\small $\pm$0.013} & 0.522{\small $\pm$0.011} \\
% & Siamese Network & 0.571{\small $\pm$0.015} & 0.508{\small $\pm$0.002} & 0.521{\small $\pm$0.000} & 0.576{\small $\pm$0.021} \\
% & Reorder & {0.634{\small $\pm$0.015}} & {0.565{\small $\pm$0.006}} & {0.546{\small $\pm$0.002}} & 0.573{\small $\pm$0.030} \\
% \hline \hline
% \end{tabular}
% }
% \label{tab:results_allmethods_weekly}
% \vspace{-0.5cm}
% \end{table}
% \renewcommand{\arraystretch}{1.0}


\renewcommand{\arraystretch}{1.2}
\begin{table}[t]
\centering
\caption{\review{Model Balanced Accuracy} of Depression Detection under Different Setups.}
% \begin{minipage}[t]{0.48\textwidth}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{c|l|C{0.21\textwidth}|C{0.21\textwidth}|C{0.21\textwidth}|C{0.21\textwidth}}
\hline \hline
\multirow{2}{*}{\textbf{Category}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \textbf{Single Dataset} & \multicolumn{3}{c}{\textbf{Cross Dataset}} \\ \cline{3-6}
 & & \textbf{Past/Future} & \textbf{Leave-One-DS-Out} & \textbf{Pre/Post-COVID} & \textbf{Overlapping Users}\\ \cline{3-6}
% & & \textbf{Bal Acc}  & \textbf{Bal Acc}  & \textbf{Bal Acc}  & \textbf{Bal Acc}  \\
\hline
Baseline & Majority & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} \\ \hdashline
\multirow{9}{*}{\makecell{Prior\\Depression\\Detection\\Model}} & Canzian \etal & 0.536{\small $\pm$0.026} & 0.498{\small $\pm$0.006} & 0.497{\small $\pm$0.003} & 0.496{\small $\pm$0.031} \\
& Saeb \etal & 0.557{\small $\pm$0.020} & 0.536{\small $\pm$0.008} & 0.519{\small $\pm$0.004} & \textbf{0.565{\small $\pm$0.039}} \\
& Farhan \etal & 0.562{\small $\pm$0.021} & 0.506{\small $\pm$0.007} & 0.500{\small $\pm$0.019} & 0.480{\small $\pm$0.013} \\
& Wahle \etal & 0.598{\small $\pm$0.020} & 0.524{\small $\pm$0.011} & 0.526{\small $\pm$0.003} & 0.512{\small $\pm$0.013} \\
& Lu \etal & 0.550{\small $\pm$0.024} & 0.531{\small $\pm$0.011} & 0.505{\small $\pm$0.007} & 0.508{\small $\pm$0.022} \\
& Wang \etal & 0.530{\small $\pm$0.020} & 0.521{\small $\pm$0.007} & 0.524{\small $\pm$0.010} & 0.532{\small $\pm$0.028} \\
& Xu \etal-I & \textbf{0.691{\small $\pm$0.018}} & 0.502{\small $\pm$0.012} & 0.519{\small $\pm$0.019} & 0.494{\small $\pm$0.013} \\
& Xu \etal-P & 0.600{\small $\pm$0.007} & 0.502{\small $\pm$0.006} & 0.508{\small $\pm$0.003} & 0.544{\small $\pm$0.009} \\
& Chikersal \etal & 0.649{\small $\pm$0.016} & \textbf{0.536{\small $\pm$0.002}} & \textbf{0.528{\small $\pm$0.024}} & 0.545{\small $\pm$0.032} \\ \hdashline
\multirow{16}{*}{\makecell{Recent\\Domain\\Generalization\\Model}} & ERM-1dCNN & 0.568{\small $\pm$0.006} & 0.510{\small $\pm$0.008} & 0.514{\small $\pm$0.006} & 0.534{\small $\pm$0.007} \\
& ERM-2dCNN & 0.533{\small $\pm$0.013} & 0.510{\small $\pm$0.006} & 0.504{\small $\pm$0.006} & 0.520{\small $\pm$0.011} \\
& ERM-LSTM & 0.565{\small $\pm$0.019} & 0.512{\small $\pm$0.006} & 0.512{\small $\pm$0.003} & 0.525{\small $\pm$0.020} \\
& ERM-Transformer & 0.584{\small $\pm$0.013} & 0.509{\small $\pm$0.008} & 0.512{\small $\pm$0.016} & 0.506{\small $\pm$0.005} \\
& ERM-Mixup & 0.568{\small $\pm$0.006} & 0.501{\small $\pm$0.008} & 0.507{\small $\pm$0.004} & 0.534{\small $\pm$0.007} \\
& IRM & 0.573{\small $\pm$0.016} & 0.506{\small $\pm$0.006} & 0.499{\small $\pm$0.000} & 0.508{\small $\pm$0.015} \\
& DANN-D & 0.526{\small $\pm$0.016} & 0.514{\small $\pm$0.004} & 0.514{\small $\pm$0.000} & 0.482{\small $\pm$0.013} \\
& DANN-P & 0.502{\small $\pm$0.002} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} & 0.486{\small $\pm$0.017} \\
& CSD-D & 0.562{\small $\pm$0.022} & 0.521{\small $\pm$0.002} & 0.512{\small $\pm$0.006} & 0.517{\small $\pm$0.025} \\
& CSD-P & 0.542{\small $\pm$0.010} & 0.511{\small $\pm$0.006} & 0.516{\small $\pm$0.000} & 0.515{\small $\pm$0.028} \\
& MLDG-D & 0.522{\small $\pm$0.013} & 0.511{\small $\pm$0.006} & 0.495{\small $\pm$0.004} & 0.519{\small $\pm$0.014} \\
& MLDG-P & 0.508{\small $\pm$0.011} & 0.510{\small $\pm$0.003} & 0.500{\small $\pm$0.003} & 0.511{\small $\pm$0.016} \\
& MASF-D & 0.505{\small $\pm$0.006} & 0.505{\small $\pm$0.001} & 0.504{\small $\pm$0.007} & 0.532{\small $\pm$0.015} \\
& MASF-P & 0.495{\small $\pm$0.007} & 0.505{\small $\pm$0.004} & 0.509{\small $\pm$0.011} & 0.530{\small $\pm$0.011} \\
& Siamese Network & 0.545{\small $\pm$0.025} & 0.509{\small $\pm$0.010} & 0.515{\small $\pm$0.002} & 0.527{\small $\pm$0.031} \\
& Reorder & \textbf{0.626{\small $\pm$0.009}} & \textbf{0.547{\small $\pm$0.008}} & \textbf{0.525{\small $\pm$0.003}} & \textbf{0.573{\small $\pm$0.030}} \\
\hline \hline
\end{tabular}
}
\label{tab:results_allmethods_weekly}
\vspace{-0.5cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg/tab_crossds_old.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[t]
\centering
\caption{\review{Model Balanced Accuracy} of Depression Detection under Different Setups.}
% \begin{minipage}[t]{0.48\textwidth}
\resizebox{1\textwidth}{!}{
\begin{tabular}[t]{c|l|C{0.21\textwidth}|C{0.21\textwidth}|C{0.21\textwidth}|C{0.21\textwidth}}
\hline \hline
\multirow{2}{*}{\textbf{Category}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \textbf{Single Dataset} & \multicolumn{3}{c}{\textbf{Cross Dataset}} \\ \cline{3-6}
 & & \textbf{Past/Future} & \textbf{Leave-One-DS-Out} & \textbf{Pre/Post-COVID} & \textbf{Overlapping Users}\\ \cline{3-6}
% & & \textbf{Bal Acc}  & \textbf{Bal Acc}  & \textbf{Bal Acc}  & \textbf{Bal Acc}  \\
\hline
Baseline & Majority & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} \\ \hdashline
\multirow{9}{*}{\makecell{Prior\\Depression\\Detection\\Model}} & Canzian \etal~\cite{canzian_trajectories_2015} & 0.527{\small $\pm$0.027} & 0.495{\small $\pm$0.006} & 0.495{\small $\pm$0.005} & 0.516{\small $\pm$0.018} \\
& Saeb \etal~\cite{saeb_mobile_2015} & 0.554{\small $\pm$0.020} & 0.534{\small $\pm$0.009} & 0.513{\small $\pm$0.002} & \textbf{0.561{\small $\pm$0.036}} \\
& Farhan \etal~\cite{farhan_behavior_2016} & 0.570{\small $\pm$0.024} & 0.521{\small $\pm$0.004} & 0.498{\small $\pm$0.032} & 0.476{\small $\pm$0.011} \\
& Wahle \etal~\cite{wahle_mobile_2016} & 0.597{\small $\pm$0.019} & 0.529{\small $\pm$0.014} & 0.527{\small $\pm$0.003} & 0.519{\small $\pm$0.018} \\
& Lu \etal~\cite{lu_joint_2018} & 0.552{\small $\pm$0.024} & 0.530{\small $\pm$0.012} & 0.505{\small $\pm$0.011} & 0.501{\small $\pm$0.016} \\
& Wang \etal~\cite{wang_tracking_2018} & 0.522{\small $\pm$0.014} & 0.517{\small $\pm$0.004} & 0.518{\small $\pm$0.009} & 0.526{\small $\pm$0.028} \\
& Xu \etal-I~\cite{xu_leveraging_2019} & \textbf{0.684{\small $\pm$0.017}} & 0.506{\small $\pm$0.011} & 0.512{\small $\pm$0.015} & 0.471{\small $\pm$0.017} \\
& Xu \etal-P~\cite{xu_leveraging_2021} & 0.578{\small $\pm$0.011} & 0.499{\small $\pm$0.007} & 0.507{\small $\pm$0.006} & 0.537{\small $\pm$0.014} \\
& Chikersal \etal~\cite{chikersal_detecting_2021} & 0.640{\small $\pm$0.010} & \textbf{0.542{\small $\pm$0.010}} & \textbf{0.531{\small $\pm$0.019}} & 0.553{\small $\pm$0.032} \\ \hdashline
\multirow{16}{*}{\makecell{Recent\\Domain\\Generalization\\Model}} & ERM-1dCNN~\cite{vapnik1999overview} & 0.620{\small $\pm$0.014} & 0.536{\small $\pm$0.007} & 0.535{\small $\pm$0.007} & 0.593{\small $\pm$0.031} \\
& ERM-2dCNN~\cite{vapnik1999overview} & 0.560{\small $\pm$0.015} & 0.527{\small $\pm$0.007} & 0.516{\small $\pm$0.006} & \textbf{0.597{\small $\pm$0.049}} \\
& ERM-LSTM~\cite{vapnik1999overview} & 0.622{\small $\pm$0.008} & 0.532{\small $\pm$0.003} & 0.509{\small $\pm$0.002} & 0.575{\small $\pm$0.026} \\
& ERM-Transformer~\cite{vapnik1999overview} & 0.530{\small $\pm$0.005} & 0.521{\small $\pm$0.006} & 0.526{\small $\pm$0.013} & 0.538{\small $\pm$0.006} \\
& ERM-Mixup~\cite{zhang_mixup_2018} & 0.620{\small $\pm$0.014} & 0.542{\small $\pm$0.005} & 0.541{\small $\pm$0.011} & 0.593{\small $\pm$0.031} \\
& IRM~\cite{arjovsky_invariant_2020} & 0.600{\small $\pm$0.015} & 0.540{\small $\pm$0.013} & 0.537{\small $\pm$0.018} & 0.578{\small $\pm$0.031} \\
& DANN-D~\cite{csurka_domain-adversarial_2017} & 0.501{\small $\pm$0.005} & 0.500{\small $\pm$0.000} & 0.507{\small $\pm$0.005} & 0.496{\small $\pm$0.003} \\
& DANN-P~\cite{csurka_domain-adversarial_2017} & 0.500{\small $\pm$0.000} & 0.499{\small $\pm$0.001} & 0.500{\small $\pm$0.000} & 0.500{\small $\pm$0.000} \\
& CSD-D~\cite{piratla_efficient_2020} & 0.612{\small $\pm$0.016} & 0.535{\small $\pm$0.010} & 0.542{\small $\pm$0.007} & 0.582{\small $\pm$0.023} \\
& CSD-P~\cite{piratla_efficient_2020} & 0.609{\small $\pm$0.018} & 0.547{\small $\pm$0.012} & 0.540{\small $\pm$0.006} & 0.577{\small $\pm$0.036} \\
& MLDG-D~\cite{li_learning_2017} & 0.507{\small $\pm$0.016} & 0.516{\small $\pm$0.003} & 0.514{\small $\pm$0.002} & 0.578{\small $\pm$0.033} \\
& MLDG-P~\cite{li_learning_2017} & 0.524{\small $\pm$0.014} & 0.506{\small $\pm$0.004} & 0.515{\small $\pm$0.002} & 0.547{\small $\pm$0.022} \\
& MASF-D~\cite{dou_domain_2019} & 0.512{\small $\pm$0.014} & 0.510{\small $\pm$0.009} & 0.498{\small $\pm$0.007} & 0.517{\small $\pm$0.005} \\
& MASF-P~\cite{dou_domain_2019} & 0.508{\small $\pm$0.022} & 0.519{\small $\pm$0.004} & 0.507{\small $\pm$0.013} & 0.522{\small $\pm$0.011} \\
& Siamese Network~\cite{koch_siamese_2015} & 0.571{\small $\pm$0.015} & 0.508{\small $\pm$0.002} & 0.521{\small $\pm$0.000} & 0.576{\small $\pm$0.021} \\
& Reorder~\cite{xu_globem_2022} & \textbf{0.634{\small $\pm$0.015}} & \textbf{0.565{\small $\pm$0.006}} & \textbf{0.546{\small $\pm$0.002}} & 0.573{\small $\pm$0.030} \\
\hline \hline
\end{tabular}
}
\label{tab:results_allmethods_weekly}
\vspace{-0.5cm}
\end{table}
\renewcommand{\arraystretch}{1.0}

==> fig_tab_alg/tab_feature_details_long.tex <==
\begin{centering}
\scriptsize
\setlength{\tabcolsep}{0.8mm}{
\begin{longtable}{l|l|l|p{0.6\textwidth}}
\caption{Description of Feature Details}
\label{tab:feature_details}
\endfirsthead
\endhead
\hline \hline
% \resizebox{1\textwidth}{!}{
% \begin{tabular}
\makecell{\textbf{Feature Type}} & \makecell{\textbf{Feature Name}} & \makecell{\textbf{Unit}} & \makecell{\textbf{Description}} \\ \hline
\multirow{35}{*}{\textbf{Location}} & hometime & minutes & Time at home. Time spent at home in minutes. Home is the most visited significant location between 8 pm and 8 am, including any pauses within a 200-meter radius. \\ \cline{2-4}
~ & disttravelled & meters & Total distance traveled over a day (flights). \\ \cline{2-4}
~ & rog & meters & The Radius of Gyration (rog) is a measure in meters of the area covered by a person over a day. A centroid is calculated for all the places (pauses) visited during a day, and a weighted distance between all the places and that centroid is computed. The weights are proportional to the time spent in each place. \\ \cline{2-4}
~ & maxdiam & meters & The maximum diameter is the largest distance between any two pauses. \\ \cline{2-4}
~ & maxhomedist & meters & The maximum distance from home in meters. \\ \cline{2-4}
~ & siglocsvisited & locations & The number of significant locations visited during the day. Significant locations are computed using k-means clustering over pauses found in the whole monitoring period. The number of clusters is found iterating k from 1 to 200 stopping until the centroids of two significant locations are within 400 meters of one another. \\ \cline{2-4}
~ & avgflightlen & meters & Mean length of all flights. \\ \cline{2-4}
~ & stdflightlen & meters & Standard deviation of the length of all flights. \\ \cline{2-4}
~ & avgflightdur & seconds & Mean duration of all flights. \\ \cline{2-4}
~ & stdflightdur & seconds & The standard deviation of the duration of all flights. \\ \cline{2-4}
~ & probpause & - & The fraction of a day spent in a pause (as opposed to a flight). \\ \cline{2-4}
~ & siglocentropy & nats & Shannon’s entropy measurement is based on the proportion of time spent at each significant location visited during a day. \\ \cline{2-4}
~ & circdnrtn & - & A continuous metric quantifying a person’s circadian routine that can take any value between 0 and 1, where 0 represents a daily routine completely different from any other sensed days and 1 a routine the same as every other sensed day. \\ \cline{2-4}
~ & wkenddayrtn & - & Same as circdnrtn but computed separately for weekends and weekdays. \\ \cline{2-4}
~ & locationvariance & meters2 & The sum of the variances of the latitude and longitude columns. \\ \cline{2-4}
~ & loglocationvariance & - & Log of the sum of the variances of the latitude and longitude columns. \\ \cline{2-4}
~ & totaldistance & meters & Total distance traveled in a time segment using the haversine formula. \\ \cline{2-4}
~ & avgspeed & km/hr & Average speed in a time segment considering only the instances labeled as Moving. This feature is 0 when the participant is stationary during a time segment. \\ \cline{2-4}
~ & varspeed & km/hr & Speed variance in a time segment considering only the instances labeled as Moving. This feature is 0 when the participant is stationary during a time segment. \\ \cline{2-4}
~ & numberofsignificantplaces & places & Number of significant locations visited. It is calculated using the DBSCAN/OPTICS clustering algorithm which takes in EPS and MIN\_SAMPLES as parameters to identify clusters. Each cluster is a significant place. \\ \cline{2-4}
~ & numberlocationtransitions & transitions & Number of movements between any two clusters in a time segment. \\ \cline{2-4}
~ & radiusgyration & meters & Quantifies the area covered by a participant. \\ \cline{2-4}
~ & timeattop1location & minutes & Time spent at the most significant location. \\ \cline{2-4}
~ & timeattop2location & minutes & Time spent at the 2nd most significant location. \\ \cline{2-4}
~ & timeattop3location & minutes & Time spent at the 3rd most significant location. \\ \cline{2-4}
~ & movingtostaticratio & - & Ratio between stationary time and total location sensed time. A lat/long coordinate pair is labeled as stationary if its speed (distance/time) to the next coordinate pair is less than 1km/hr. A higher value represents a more stationary routine. \\ \cline{2-4}
~ & outlierstimepercent & - & Ratio between the time spent in non-significant clusters divided by the time spent in all clusters (stationary time. Only stationary samples are clustered). A higher value represents more time spent in non-significant clusters. \\ \cline{2-4}
~ & maxlengthstayatclusters & minutes & Maximum time spent in a cluster (significant location). \\ \cline{2-4}
~ & minlengthstayatclusters & minutes & Minimum time spent in a cluster (significant location). \\ \cline{2-4}
~ & avglengthstayatclusters & minutes & Average time spent in a cluster (significant location). \\ \cline{2-4}
~ & stdlengthstayatclusters & minutes & Standard deviation of time spent in a cluster (significant location). \\ \cline{2-4}
~ & locationentropy & nats & Shannon Entropy computed over the row count of each cluster (significant location), it is higher the more rows belong to a cluster (i.e., the more time a participant spent at a significant location). \\ \cline{2-4}
~ & normalizedlocationentropy & nats & Shannon Entropy computed over the row count of each cluster (significant location) divided by the number of clusters; it is higher the more rows belong to a cluster (i.e., the more time a participant spent at a significant location). \\ \cline{2-4}
~ & timeathome & minutes & Time spent at home. \\ \cline{2-4}
~ & timeat [PLACE] & minutes & Time spent at [PLACE], which can be living, exercise, study, greens. \\ \hline
PhoneUsage & sumduration & minutes & Total duration of all unlock episodes. \\ \cline{2-4}
~ & maxduration & minutes & Longest duration of any unlock episode. \\ \cline{2-4}
~ & minduration & minutes & Shortest duration of any unlock episode. \\ \cline{2-4}
~ & avgduration & minutes & Average duration of all unlock episodes. \\ \cline{2-4}
~ & stdduration & minutes & Standard deviation duration of all unlock episodes. \\ \cline{2-4}
~ & countepisode & episodes & Number of all unlock episodes. \\ \cline{2-4}
~ & firstuseafter & minutes & Minutes until the first unlock episode. \\ \cline{2-4}
~ & sumduration [PLACE] & minutes & Total duration of all unlock episodes. [PLACE] can be living, exercise, study, greens. Same below. \\ \cline{2-4}
~ & maxduration [PLACE] & minutes & Longest duration of any unlock episode. \\ \cline{2-4}
~ & minduration [PLACE] & minutes & Shortest duration of any unlock episode. \\ \cline{2-4}
~ & avgduration [PLACE] & minutes & Average duration of all unlock episodes. \\ \cline{2-4}
~ & stdduration [PLACE] & minutes & Standard deviation duration of all unlock episodes. \\ \cline{2-4}
~ & countepisode [PLACE] & episodes & Number of all unlock episodes. \\ \cline{2-4}
~ & firstuseafter [PLACE] & minutes & Minutes until the first unlock episode. \\ \hline
Call & count & calls & Number of calls of a particular call\_type [incoming/outgoing] occurred during a particular time\_segment. \\ \cline{2-4}
~ & distinctcontacts & contacts & Number of distinct contacts that are associated with a particular call\_type for a particular time\_segment. \\ \cline{2-4}
~ & meanduration & seconds & The mean duration of all calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
~ & sumduration & seconds & The sum of the duration of all calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
~ & minduration & seconds & The duration of the shortest call of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
~ & maxduration & seconds & The duration of the longest call of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
~ & stdduration & seconds & The standard deviation of the duration of all the calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
~ & modeduration & seconds & The mode of the duration of all the calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
~ & entropyduration & nats & The estimate of the Shannon entropy for the the duration of all the calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
~ & timefirstcall & minutes & The time in minutes between 12:00am (midnight) and the first call of call\_type. \\ \cline{2-4}
~ & timelastcall & minutes & The time in minutes between 12:00am (midnight) and the last call of call\_type. \\ \cline{2-4}
~ & countmostfrequentcontact & calls & The number of calls of a particular call\_type during a particular time\_segment of the most frequent contact throughout the monitored period. \\ \hline
Bluetooth & countscans & scans & Number of scans (rows) from the devices sensed during a time segment instance. The more scans a bluetooth device has the longer it remained within range of the participant’s phone. \\ \cline{2-4}
~ & uniquedevices & devices & Number of unique bluetooth devices sensed during a time segment instance as identified by their hardware addresses (bt\_address). \\ \cline{2-4}
~ & meanscans & scans & Mean of the scans of every sensed device within each time segment instance. \\ \cline{2-4}
~ & stdscans & scans & Standard deviation of the scans of every sensed device within each time segment instance. \\ \cline{2-4}
~ & \makecell[l]{countscansmostfrequent\\devicewithinsegments} & scans & Number of scans of the most sensed device within each time segment instance. \\ \cline{2-4}
~ & \makecell[l]{countscansleastfrequent\\devicewithinsegments} & scans & Number of scans of the least sensed device within each time segment instance. \\ \cline{2-4}
~ & \makecell[l]{countscansmostfrequent\\deviceacrosssegments} & scans & Number of scans of the most sensed device across time segment instances of the same type. \\ \cline{2-4}
~ & \makecell[l]{countscansleastfrequent\\deviceacrosssegments} & scans & Number of scans of the least sensed device across time segment instances of the same type per device. \\ \cline{2-4}
~ & \makecell[l]{countscansmostfrequent\\deviceacrossdataset} & scans & Number of scans of the most sensed device across the entire dataset of every participant. \\ \cline{2-4}
~ & \makecell[l]{countscansleastfrequent\\deviceacrossdataset} & scans & Number of scans of the least sensed device across the entire dataset of every participant. \\ \hline
Physical Activity & maxsumsteps & steps & The maximum daily step count during a time segment. \\ \cline{2-4}
~ & minsumsteps & steps & The minimum daily step count during a time segment. \\ \cline{2-4}
~ & avgsumsteps & steps & The average daily step count during a time segment. \\ \cline{2-4}
~ & mediansumsteps & steps & The median of daily step count during a time segment. \\ \cline{2-4}
~ & stdsumsteps & steps & The standard deviation of daily step count during a time segment. \\ \cline{2-4}
~ & sumsteps & steps & The total step count during a time segment. \\ \cline{2-4}
~ & maxsteps & steps & The maximum step count during a time segment. \\ \cline{2-4}
~ & minsteps & steps & The minimum step count during a time segment. \\ \cline{2-4}
~ & avgsteps & steps & The average step count during a time segment. \\ \cline{2-4}
~ & stdsteps & steps & The standard deviation of step count during a time segment. \\ \cline{2-4}
~ & countepisodesedentarybout & bouts & Number of sedentary bouts during a time segment. \\ \cline{2-4}
~ & sumdurationsedentarybout & minutes & Total duration of all sedentary bouts during a time segment. \\ \cline{2-4}
~ & maxdurationsedentarybout & minutes & The maximum duration of any sedentary bout during a time segment. \\ \cline{2-4}
~ & mindurationsedentarybout & minutes & The minimum duration of any sedentary bout during a time segment. \\ \cline{2-4}
~ & avgdurationsedentarybout & minutes & The average duration of sedentary bouts during a time segment. \\ \cline{2-4}
~ & stddurationsedentarybout & minutes & The standard deviation of the duration of sedentary bouts during a time segment. \\ \cline{2-4}
~ & countepisodeactivebout & bouts & Number of active bouts during a time segment. \\ \cline{2-4}
~ & sumdurationactivebout & minutes & Total duration of all active bouts during a time segment. \\ \cline{2-4}
~ & maxdurationactivebout & minutes & The maximum duration of any active bout during a time segment. \\ \cline{2-4}
~ & mindurationactivebout & minutes & The minimum duration of any active bout during a time segment. \\ \cline{2-4}
~ & avgdurationactivebout & minutes & The average duration of active bouts during a time segment. \\ \cline{2-4}
~ & stddurationactivebout & minutes & The standard deviation of the duration of active bouts during a time segment. \\ \hline
Sleep & \makecell[l]{countepisode\\ {[}LEVEL{]}{[}TYPE{]}} & episodes & Number of [LEVEL][TYPE] sleep episodes. [LEVEL] is one of awake and asleep and [TYPE] is one of main, nap, and all. Same below. \\ \cline{2-4}
~ & \makecell[l]{sumduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Total duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
~ & \makecell[l]{maxduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Longest duration of any [LEVEL][TYPE] sleep episode. \\ \cline{2-4}
~ & \makecell[l]{minduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Shortest duration of any [LEVEL][TYPE] sleep episode. \\ \cline{2-4}
~ & \makecell[l]{avgduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Average duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
~ & \makecell[l]{medianduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Median duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
~ & \makecell[l]{stdduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Standard deviation duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
~ & \makecell[l]{firstwaketime\\ {[}TYPE{]}} & minutes & First wake time for a certain sleep type during a time segment. Wake time is number of minutes after midnight of a sleep episode’s end time. \\ \cline{2-4}
~ & \makecell[l]{lastwaketime\\ {[}TYPE{]}} & minutes & Last wake time for a certain sleep type during a time segment. Wake time is number of minutes after midnight of a sleep episode’s end time. \\ \cline{2-4}
~ & \makecell[l]{firstbedtime\\ {[}TYPE{]}} & minutes & First bedtime for a certain sleep type during a time segment. Bedtime is number of minutes after midnight of a sleep episode’s start time. \\ \cline{2-4}
~ & \makecell[l]{lastbedtime\\ {[}TYPE{]}} & minutes & Last bedtime for a certain sleep type during a time segment. Bedtime is number of minutes after midnight of a sleep episode’s start time. \\ \cline{2-4}
~ & \makecell[l]{countepisode\\ {[}TYPE{]}} & episodes & Number of sleep episodes for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{avgefficiency\\ {[}TYPE{]}} & scores & Average sleep efficiency for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{sumdurationafterwakeup\\ {[}TYPE{]}} & minutes & Total duration the user stayed in bed after waking up for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{sumdurationasleep\\ {[}TYPE{]}} & minutes & Total sleep duration for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{sumdurationawake\\ {[}TYPE{]}} & minutes & Total duration the user stayed awake but still in bed for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{sumdurationtofallasleep\\ {[}TYPE{]}} & minutes & Total duration the user spent to fall asleep for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{sumdurationinbed\\ {[}TYPE{]}} & minutes & Total duration the user stayed in bed (sumdurationtofallasleep + sumdurationawake + sumdurationasleep + sumdurationafterwakeup) for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{avgdurationafterwakeup\\ {[}TYPE{]}} & minutes & Average duration the user stayed in bed after waking up for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{avgdurationasleep\\ {[}TYPE{]}} & minutes & Average sleep duration for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{avgdurationawake\\ {[}TYPE{]}} & minutes & Average duration the user stayed awake but still in bed for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{avgdurationtofallasleep\\ {[}TYPE{]}} & minutes & Average duration the user spent to fall asleep for a certain sleep type during a time segment. \\ \cline{2-4}
~ & \makecell[l]{avgdurationinbed\\ {[}TYPE{]}} & minutes & Average duration the user stayed in bed (sumdurationtofallasleep + sumdurationawake + sumdurationasleep + sumdurationafterwakeup) for a certain sleep type during a time segment. \\ \cline{2-4}
% }
\end{longtable}}
\end{centering}

==> fig_tab_alg/tab_feature_details_old.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table}[h!]
\centering
\caption{Description of Location Features. Texts taken from \href{https://www.rapids.science/1.6/}{RAPIDS} with courtesy, the same below.}
\label{tab:feature_details_location}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{C{0.15\textwidth}|L{0.28\textwidth}|L{0.1\textwidth}|L{0.8\textwidth}}
\hline \hline
\makecell{\textbf{Feature Type}} & \makecell{\textbf{Feature Name}} & \makecell{\textbf{Unit}} & \makecell{\textbf{Description}} \\ \hline
\multirow{50}{*}{\makecell{\textbf{Location}}} & hometime & minutes & Time at home. Time spent at home in minutes. Home is the most visited significant location between 8 pm and 8 am, including any pauses within a 200-meter radius. \\ \cline{2-4}
& disttravelled & meters & Total distance traveled over a day (flights). \\ \cline{2-4}
& rog & meters & The Radius of Gyration (rog) is a measure in meters of the area covered by a person over a day. A centroid is calculated for all the places (pauses) visited during a day, and a weighted distance between all the places and that centroid is computed. The weights are proportional to the time spent in each place. \\ \cline{2-4}
& maxdiam & meters & The maximum diameter is the largest distance between any two pauses. \\ \cline{2-4}
& maxhomedist & meters & The maximum distance from home in meters. \\ \cline{2-4}
& siglocsvisited & locations & The number of significant locations visited during the day. Significant locations are computed using k-means clustering over pauses found in the whole monitoring period. The number of clusters is found iterating k from 1 to 200 stopping until the centroids of two significant locations are within 400 meters of one another. \\ \cline{2-4}
& avgflightlen & meters & Mean length of all flights. \\ \cline{2-4}
& stdflightlen & meters & Standard deviation of the length of all flights. \\ \cline{2-4}
& avgflightdur & seconds & Mean duration of all flights. \\ \cline{2-4}
& stdflightdur & seconds & The standard deviation of the duration of all flights. \\ \cline{2-4}
& probpause & - & The fraction of a day spent in a pause (as opposed to a flight). \\ \cline{2-4}
& siglocentropy & nats & Shannon’s entropy measurement is based on the proportion of time spent at each significant location visited during a day. \\ \cline{2-4}
& circdnrtn & - & A continuous metric quantifying a person’s circadian routine that can take any value between 0 and 1, where 0 represents a daily routine completely different from any other sensed days and 1 a routine the same as every other sensed day. \\ \cline{2-4}
& wkenddayrtn & - & Same as circdnrtn but computed separately for weekends and weekdays. \\ \cline{2-4}
& locationvariance & meters2 & The sum of the variances of the latitude and longitude columns. \\ \cline{2-4}
& loglocationvariance & - & Log of the sum of the variances of the latitude and longitude columns. \\ \cline{2-4}
& totaldistance & meters & Total distance traveled in a time segment using the haversine formula. \\ \cline{2-4}
& avgspeed & km/hr & Average speed in a time segment considering only the instances labeled as Moving. This feature is 0 when the participant is stationary during a time segment. \\ \cline{2-4}
& varspeed & km/hr & Speed variance in a time segment considering only the instances labeled as Moving. This feature is 0 when the participant is stationary during a time segment. \\ \cline{2-4}
& numberofsignificantplaces & places & Number of significant locations visited. It is calculated using the DBSCAN/OPTICS clustering algorithm which takes in EPS and MIN\_SAMPLES as parameters to identify clusters. Each cluster is a significant place. \\ \cline{2-4}
& numberlocationtransitions & transitions & Number of movements between any two clusters in a time segment. \\ \cline{2-4}
& radiusgyration & meters & Quantifies the area covered by a participant. \\ \cline{2-4}
& timeattop1location & minutes & Time spent at the most significant location. \\ \cline{2-4}
& timeattop2location & minutes & Time spent at the 2nd most significant location. \\ \cline{2-4}
& timeattop3location & minutes & Time spent at the 3rd most significant location. \\ \cline{2-4}
& movingtostaticratio & - & Ratio between stationary time and total location sensed time. A lat/long coordinate pair is labeled as stationary if its speed (distance/time) to the next coordinate pair is less than 1km/hr. A higher value represents a more stationary routine. \\ \cline{2-4}
& outlierstimepercent & - & Ratio between the time spent in non-significant clusters divided by the time spent in all clusters (stationary time. Only stationary samples are clustered). A higher value represents more time spent in non-significant clusters. \\ \cline{2-4}
& maxlengthstayatclusters & minutes & Maximum time spent in a cluster (significant location). \\ \cline{2-4}
& minlengthstayatclusters & minutes & Minimum time spent in a cluster (significant location). \\ \cline{2-4}
& avglengthstayatclusters & minutes & Average time spent in a cluster (significant location). \\ \cline{2-4}
& stdlengthstayatclusters & minutes & Standard deviation of time spent in a cluster (significant location). \\ \cline{2-4}
& locationentropy & nats & Shannon Entropy computed over the row count of each cluster (significant location), it is higher the more rows belong to a cluster (i.e., the more time a participant spent at a significant location). \\ \cline{2-4}
& normalizedlocationentropy & nats & Shannon Entropy computed over the row count of each cluster (significant location) divided by the number of clusters; it is higher the more rows belong to a cluster (i.e., the more time a participant spent at a significant location). \\ \cline{2-4}
& timeathome & minutes & Time spent at home. \\ \cline{2-4}
& timeat [PLACE] & minutes & Time spent at [PLACE], which can be living, exercise, study, greens. \\
\hline \hline
\end{tabular}
\vspace{-1cm}
}
\end{table}

\newpage

\begin{table}[h!]
\centering
\caption{Description of Phone Usage, Call, and Bluetooth Features}
\label{tab:feature_details_screen_call_bluetooth}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{C{0.15\textwidth}|L{0.28\textwidth}|L{0.1\textwidth}|L{0.8\textwidth}}
\hline \hline
\makecell{\textbf{Feature Type}} & \makecell{\textbf{Feature Name}} & \makecell{\textbf{Unit}} & \makecell{\textbf{Description}} \\ \hline
\multirow{15}{*}{\makecell{\textbf{Phone Usage}}} & sumduration & minutes & Total duration of all unlock episodes. \\ \cline{2-4}
& maxduration & minutes & Longest duration of any unlock episode. \\ \cline{2-4}
& minduration & minutes & Shortest duration of any unlock episode. \\ \cline{2-4}
& avgduration & minutes & Average duration of all unlock episodes. \\ \cline{2-4}
& stdduration & minutes & Standard deviation duration of all unlock episodes. \\ \cline{2-4}
& countepisode & episodes & Number of all unlock episodes. \\ \cline{2-4}
& firstuseafter & minutes & Minutes until the first unlock episode. \\ \cline{2-4}
& sumduration [PLACE] & minutes & Total duration of all unlock episodes. [PLACE] can be living, exercise, study, greens. Same below. \\ \cline{2-4}
& maxduration [PLACE] & minutes & Longest duration of any unlock episode. \\ \cline{2-4}
& minduration [PLACE] & minutes & Shortest duration of any unlock episode. \\ \cline{2-4}
& avgduration [PLACE] & minutes & Average duration of all unlock episodes. \\ \cline{2-4}
& stdduration [PLACE] & minutes & Standard deviation duration of all unlock episodes. \\ \cline{2-4}
& countepisode [PLACE] & episodes & Number of all unlock episodes. \\ \cline{2-4}
& firstuseafter [PLACE] & minutes & Minutes until the first unlock episode. \\ \hline
\multirow{20}{*}{\makecell{\textbf{Call}}} & count & calls & Number of calls of a particular call\_type (either incoming or outgoing, same below) occurred during a particular time\_segment. \\ \cline{2-4}
& distinctcontacts & contacts & Number of distinct contacts that are associated with a particular call\_type for a particular time\_segment. \\ \cline{2-4}
& meanduration & seconds & The mean duration of all calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
& sumduration & seconds & The sum of the duration of all calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
& minduration & seconds & The duration of the shortest call of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
& maxduration & seconds & The duration of the longest call of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
& stdduration & seconds & The standard deviation of the duration of all the calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
& modeduration & seconds & The mode of the duration of all the calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
& entropyduration & nats & The estimate of the Shannon entropy for the the duration of all the calls of a particular call\_type during a particular time\_segment. \\ \cline{2-4}
& timefirstcall & minutes & The time in minutes between 12:00am (midnight) and the first call of call\_type. \\ \cline{2-4}
& timelastcall & minutes & The time in minutes between 12:00am (midnight) and the last call of call\_type. \\ \cline{2-4}
& countmostfrequentcontact & calls & The number of calls of a particular call\_type during a particular time\_segment of the most frequent contact throughout the monitored period. \\ \hline
\multirow{17}{*}{\makecell{\textbf{Bluetooth}}} & countscans & scans & Number of scans (rows) from the devices sensed during a time segment instance. The more scans a bluetooth device has the longer it remained within range of the participant’s phone. \\ \cline{2-4}
& uniquedevices & devices & Number of unique bluetooth devices sensed during a time segment instance as identified by their hardware addresses (bt\_address). \\ \cline{2-4}
& meanscans & scans & Mean of the scans of every sensed device within each time segment instance. \\ \cline{2-4}
& stdscans & scans & Standard deviation of the scans of every sensed device within each time segment instance. \\ \cline{2-4}
& \makecell[l]{countscansmostfrequent\\devicewithinsegments} & scans & Number of scans of the most sensed device within each time segment instance. \\ \cline{2-4}
& \makecell[l]{countscansleastfrequent\\devicewithinsegments} & scans & Number of scans of the least sensed device within each time segment instance. \\ \cline{2-4}
& \makecell[l]{countscansmostfrequent\\deviceacrosssegments} & scans & Number of scans of the most sensed device across time segment instances of the same type. \\ \cline{2-4}
& \makecell[l]{countscansleastfrequent\\deviceacrosssegments} & scans & Number of scans of the least sensed device across time segment instances of the same type per device. \\ \cline{2-4}
& \makecell[l]{countscansmostfrequent\\deviceacrossdataset} & scans & Number of scans of the most sensed device across the entire dataset of every participant. \\ \cline{2-4}
& \makecell[l]{countscansleastfrequent\\deviceacrossdataset} & scans & Number of scans of the least sensed device across the entire dataset of every participant. \\
\hline \hline
\end{tabular}
}
\end{table}

\newpage

\begin{table}[h!]
\centering
\caption{Description of Physical Activity and Sleep Features}
\label{tab:feature_details_step_sleep}
\resizebox{0.98\textwidth}{!}{
\begin{tabular}{C{0.15\textwidth}|L{0.28\textwidth}|L{0.1\textwidth}|L{0.8\textwidth}}
\hline \hline
\makecell{\textbf{Feature Type}} & \makecell{\textbf{Feature Name}} & \makecell{\textbf{Unit}} & \makecell{\textbf{Description}} \\ \hline
\multirow{18}{*}{\makecell{\textbf{Physical} \\ \textbf{Activity}}} & maxsumsteps & steps & The maximum daily step count during a time segment. \\ \cline{2-4}
& minsumsteps & steps & The minimum daily step count during a time segment. \\ \cline{2-4}
& avgsumsteps & steps & The average daily step count during a time segment. \\ \cline{2-4}
& mediansumsteps & steps & The median of daily step count during a time segment. \\ \cline{2-4}
& stdsumsteps & steps & The standard deviation of daily step count during a time segment. \\ \cline{2-4}
& sumsteps & steps & The total step count during a time segment. \\ \cline{2-4}
& maxsteps & steps & The maximum step count during a time segment. \\ \cline{2-4}
& minsteps & steps & The minimum step count during a time segment. \\ \cline{2-4}
& avgsteps & steps & The average step count during a time segment. \\ \cline{2-4}
& countepisodesedentarybout & bouts & Number of sedentary bouts during a time segment. \\ \cline{2-4}
& sumdurationsedentarybout & minutes & Total duration of all sedentary bouts during a time segment. \\ \cline{2-4}
& maxdurationsedentarybout & minutes & The maximum duration of any sedentary bout during a time segment. \\ \cline{2-4}
& mindurationsedentarybout & minutes & The minimum duration of any sedentary bout during a time segment. \\ \cline{2-4}
& avgdurationsedentarybout & minutes & The average duration of sedentary bouts during a time segment. \\ \cline{2-4}
& stddurationsedentarybout & minutes & The standard deviation of the duration of sedentary bouts during a time segment. \\ \cline{2-4}
& countepisodeactivebout & bouts & Number of active bouts during a time segment. \\ \cline{2-4}
& sumdurationactivebout & minutes & Total duration of all active bouts during a time segment. \\ \cline{2-4}
& maxdurationactivebout & minutes & The maximum duration of any active bout during a time segment. \\ \cline{2-4}
& mindurationactivebout & minutes & The minimum duration of any active bout during a time segment. \\ \cline{2-4}
& avgdurationactivebout & minutes & The average duration of active bouts during a time segment. \\ \cline{2-4}
& stddurationactivebout & minutes & The standard deviation of the duration of active bouts during a time segment. \\ \hline
\multirow{40}{*}{\makecell{\textbf{Sleep}}} & \makecell[l]{countepisode\\ {[}LEVEL{]}{[}TYPE{]}} & episodes & Number of [LEVEL][TYPE] sleep episodes. [LEVEL] is one of awake and asleep and [TYPE] is one of main, nap, and all. Same below. \\ \cline{2-4}
& \makecell[l]{sumduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Total duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
& \makecell[l]{maxduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Longest duration of any [LEVEL][TYPE] sleep episode. \\ \cline{2-4}
& \makecell[l]{minduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Shortest duration of any [LEVEL][TYPE] sleep episode. \\ \cline{2-4}
& \makecell[l]{avgduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Average duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
& \makecell[l]{medianduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Median duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
& \makecell[l]{stdduration\\ {[}LEVEL{]}{[}TYPE{]}} & minutes & Standard deviation duration of all [LEVEL][TYPE] sleep episodes. \\ \cline{2-4}
& \makecell[l]{firstwaketime {[}TYPE{]}} & minutes & First wake time for a certain sleep type during a time segment. Wake time is number of minutes after midnight of a sleep episode’s end time. \\ \cline{2-4}
& \makecell[l]{lastwaketime {[}TYPE{]}} & minutes & Last wake time for a certain sleep type during a time segment. Wake time is number of minutes after midnight of a sleep episode’s end time. \\ \cline{2-4}
& \makecell[l]{firstbedtime {[}TYPE{]}} & minutes & First bedtime for a certain sleep type during a time segment. Bedtime is number of minutes after midnight of a sleep episode’s start time. \\ \cline{2-4}
& \makecell[l]{lastbedtime {[}TYPE{]}} & minutes & Last bedtime for a certain sleep type during a time segment. Bedtime is number of minutes after midnight of a sleep episode’s start time. \\ \cline{2-4}
& \makecell[l]{countepisode {[}TYPE{]}} & episodes & Number of sleep episodes for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{avgefficiency {[}TYPE{]}} & scores & Average sleep efficiency for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{sumdurationafterwakeup\\ {[}TYPE{]}} & minutes & Total duration the user stayed in bed after waking up for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{sumdurationasleep\\ {[}TYPE{]}} & minutes & Total sleep duration for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{sumdurationawake\\ {[}TYPE{]}} & minutes & Total duration the user stayed awake but still in bed for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{sumdurationtofallasleep\\ {[}TYPE{]}} & minutes & Total duration the user spent to fall asleep for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{sumdurationinbed\\ {[}TYPE{]}} & minutes & Total duration the user stayed in bed (sumdurationtofallasleep + sumdurationawake + sumdurationasleep + sumdurationafterwakeup) for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{avgdurationafterwakeup\\ {[}TYPE{]}} & minutes & Average duration the user stayed in bed after waking up for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{avgdurationasleep\\ {[}TYPE{]}} & minutes & Average sleep duration for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{avgdurationawake\\ {[}TYPE{]}} & minutes & Average duration the user stayed awake but still in bed for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{avgdurationtofallasleep\\ {[}TYPE{]}} & minutes & Average duration the user spent to fall asleep for a certain sleep type during a time segment. \\ \cline{2-4}
& \makecell[l]{avgdurationinbed\\ {[}TYPE{]}} & minutes & Average duration the user stayed in bed (sumdurationtofallasleep + sumdurationawake + sumdurationasleep + sumdurationafterwakeup) for a certain sleep type during a time segment. \\
\hline \hline
\end{tabular}
}
\end{table}
\renewcommand{\arraystretch}{1.0}
\vspace{-0.2cm}
PS. One limitation of our physical activity and sleep feature data comes from a Fitbit issue: If the data on the wearable device is not synced with the smartphone over a few days, it would trigger some internal space-saving strategy to discard low-level details and only contain high-level summary data, leading to information loss and affecting feature correctness. This would be reflected by the missing features (\eg small or missing \texttt{countepisodeactivebout}), which is not common in our datasets.

==> fig_tab_alg/tab_survey_details_display_noref.tex <==
\begin{centering}
    \scriptsize
    \setlength{\tabcolsep}{0.8mm}{
    \begin{longtable}{c|m{0.45\textwidth}|c|c|c}
    \caption{Description of Survey Scales}
    \label{tab:survey_details}
    \endfirsthead
    \endhead
    \hline \hline
    \multicolumn{1}{c|}{\textbf{Scale Name \& Abbreviation}} & \multicolumn{1}{c|}{\textbf{Short Description}} & \multicolumn{1}{c|}{\textbf{Scoring Range}} & \multicolumn{1}{c|}{\textbf{Year}} & \multicolumn{1}{c}{\makecell[c]{\textbf{Collection}\\ \textbf{Time}}} \\\hline
        %Short-form UCLA Loneliness Scale 
        \makecell{UCLA \\ Short-form UCLA\\Loneliness Scale} & A 10-item scale measuring one's subjective feelings of loneliness as well as social isolation. Items 2, 6, 10, 11, 13, 14, 16, 18, 19, and 20 of the original scale are included in the short form. Higher values indicate more subjective loneliness. & 10 - 40 & \multirow{35}{*}{1,2,3,4} & \multirow{35}{*}{pre, post} \\\cline{1-3}
        \makecell{SocialFit  \\ Sense of Social \\ and Academic Fit Scale} & A 17-item scale measuring the sense of social and academic fit of students at the institution where this study was conducted. Higher values indicate higher feelings of belongings. & 17 - 119 &  &   \\\cline{1-3}
        \makecell{2-Way SSS \\2-Way Social\\Support Scale} & A 21-item scale measuring social supports from four aspects (a) giving emotional support, (b) giving instrumental support, (c) receiving emotional support, and (d) receiving instrumental support. Higher values indicate more social support. & \makecell[c]{(a) 0 - 25 \\ (b) 0 - 25 \\ (c) 0 - 35 \\ (d) 0 - 20} &   &  \\\cline{1-3}
        \makecell{PSS \\ Perceived Stress Scale} & A 14-item scale used to assess stress levels during the last month. Note that Year 1 used the 10-item version. Higher values indicate more perceived stress. & \makecell[c]{0 - 56 (Year 2,3,4)\\ 0 - 40 (Year 1)} &  &  \\\cline{1-3}
        \makecell{ERQ  \\ Emotion Regulation \\Questionnaire} & A 10-item scale assessing individual differences in the habitual use of two emotion regulation strategies: (a) cognitive reappraisal and (b) expressive suppression. Higher scores indicate more habitual use of reappraisal/suppression. & \makecell[c]{(a) 1 - 7 \\ (b) 1 - 7}&  &  \\\cline{1-3}
        \makecell{BRS  \\ Brief Resilience Scale} & A 6-item scale assessing the ability to bounce back or recover from stress. Higher scores indicate more resilient from stress. & 1 - 5 &  &  \\\cline{1-3}
        \makecell{CHIPS \\ Cohen-Hoberman Inventory\\ of Physical Symptoms} & A 33-item scale measuring the perceived burden from physical symptoms, and resulting psychological effect during the past 2 weeks. Higher values indicate more perceived burden from physical symptoms. & 0 - 132 &  &  \\\cline{1-3}
        \makecell{STAI \\ State-Trait Anxiety \\ Inventory for Adults} & A 20-item scale measuring State-Trait anxiety. Year 1 used the State version, while other years used the Trait version. Higher values indicate higher anxiety. & 20 - 80 & & \\\cline{1-3}
        \makecell{CES-D \\ Center for Epidemiologic\\ Studies Depression Scale\\ Cole version} & A 10-item scale measuring current level of depressive symptomatology, with emphasis on the affective component, depressed mood. Year 2 used the 9-item version. Higher scores indicate more depressive symptoms. & \makecell[c]{0 - 30 (Year 1,3,4) \\ 0 - 27 (Year 2)} &  &  \\\cline{1-3}
        \makecell{BDI2  \\ Beck Depression \\ Inventory-II} & A 21-item  detect depressive symptoms. Higher values indicate more depressive symptoms. 0-13: minimal to none, 14-19: mild, 20-28: moderate and 26-63: severe. & \makecell[c]{0 - 63} &  &  \\\cline{1-3}
        \makecell{MAAS  \\ Mindful Attention \\ Awareness Scale} & A 15-item scale assessing a core characteristic of  mindfulness. Year 1 used a 7-item version, while other years used the full version. Higher values indicate higher mindfulness. & 1 - 6 &  &  \\\hline
        \makecell{BFI10 \\The Big-Five Inventory-10} & A 10-item scale measuring the Big Five personality traits Extroversion, Agreeableness, Conscientiousness, Emotional Stability, and Openness. The higher the score, the greater the tendency of the corresponding personality. & 1 - 5  & 1,2,3,4 & pre \\\hline
        %RRQ  & \makecell[l]{A 24-item scale evaluating the ruminative and reflective types of private self-consciousness. Higher values indicate more tendency of ruminative/ref-\\lective types of private self-attentiveness.} & 1 - 5 & \multirow{9}{*}{2,3,4} & \multirow{9}{*}{pre, post} \\\cline{1-3}
        \makecell{Brief-COPE \\ Brief Coping Orientation\\to Problems Experienced} & A 28-item scale measuring (a) adaptive and (b) maladaptive ways to cope with a stressful life event. Higher values indicate more effective/ineffective ways to cope with a stressful life event. & \makecell[c]{(a): 0 - 3 \\ (b): 0 - 3} & \multirow{18}{*}{2,3,4} & \multirow{18}{*}{pre, post} \\\cline{1-3}
        \makecell{GQ \\ Gratitude Questionnaire} & A 6-item scale assessing individual differences in the proneness to experience gratitude in daily life. Higher scores indicate a greater tendency to experience gratitude.  & 6 - 42 &  &  \\\cline{1-3}
        \makecell{FSPWB \\Flourishing Scale \\ \& Psychological \\ Well-Being Scale} & An 8-item scale measuring the psychological well-being. Higher scores indicate a person with ``more psychological resources and mental strengths''. & 8 - 56 &  &  \\\cline{1-3}
        \makecell{EDS \\ Everyday Discrimination\\ Scale}& A 9-item scale assessing everyday discrimination. Higher values indicate more frequent experience of discrimination. &  0 - 45 &  &  \\\cline{1-3}
        %\makecell{MED \\ Major Experiences \\ of Discrimination} & A 4-item scale assessing major experiences of discrimination. Higher scores indicate more acute experiences as well as the more recent the experiences have been. & \makecell[c]{0 - 12} &  &  \\\cline{1-3}
        \makecell{CEDH \\ Chronic Work Discrimination\\ and Harassment} & A 12-item scale assessing experiences of discrimination in educational  settings. Higher values indicate more frequent experience of discrimination in the work environment. & 0 - 60 &  &  \\\cline{1-3}
        \makecell{B-YAACQ \\The Brief Young Adult \\ Alcohol Consequences\\ Questionnaire (optional)} & A 24-item scale measuring the alcohol problem severity continuum in college students. Higher values indicates more severe alcohol problems. & 0 - 24 &  & \\\hline
        %PTSD  & \makecell[l]{A 33-item scale assessing the posttraumatic stress \\ disorder in corresponding to the DSM-5.} & 0(Not at all) - 4(Extremely) & 2,3,4 & pre \\\hline
        \makecell{PHQ-4 \\Patient Health \\Questionnaire 4} & A 4-item scale assessing (a) mental health, (b) anxiety, and (c) depression. Higher values indicate higher risk of mental health, anxiety, and depression. & \makecell[c]{(a): 0 - 12 \\ (b): 0 - 6 \\ (c): 0 - 6} & \multirow{7}{*}{2,3,4} & \multirow{7}{*}{\makecell{Weekly\\EMA}} \\\cline{1-3}
        \makecell{PSS-4 \\Perceived Stress Scale 4}& A 4-item scale assessing stress levels during the last month. Higher values indicates more perceived stress. & 0 - 16 &  &  \\\cline{1-3}
        \makecell{PANAS \\Positive and Negative\\Affect Schedule} & A 10-item scale measuring the level of (a) positive and (b) negative affects. Higher values indicates larger extent. & \makecell[c]{(a): 0 - 20 \\ (b): 0 - 20} &  &  \\
    \hline \hline
    \end{longtable}}
\end{centering}
